Finite-Function-Encoding Quantum States

We introduce finite-function-encoding (FFE) states which encode arbitrary $d$-valued logic functions, i.e., multivariate functions over the ring of integers modulo $d$, and investigate some of their structural properties. We also point out some differences between polynomial and non-polynomial function encoding states: The former can be associated to graphical objects, that we dub tensor-edge hypergraphs (TEH), which are a generalization of hypergraphs with a tensor attached to each hyperedge encoding the coefficients of the different monomials. To complete the framework, we also introduce a notion of finite-function-encoding Pauli (FP) operators, which correspond to elements of what is known as the generalized symmetric group in mathematics. First, using this machinery, we study the stabilizer group associated to FFE states and observe how qudit hypergraph states introduced in arXiv:1612.06418v2 admit stabilizers of a particularly simpler form. Afterwards, we investigate the classification of FFE states under local unitaries (LU), and, after showing the complexity of this problem, we focus on the case of bipartite states and especially on the classification under local FP operations (LFP). We find all LU and LFP classes for two qutrits and two ququarts and study several other special classes, pointing out the relation between maximally entangled FFE states and complex Butson-type Hadamard matrices. Our investigation showcases also the relation between the properties of FFE states, especially their LU classification, and the theory of finite rings over the integers.

==> docs/dim3.tex <==
In this qutrit case this results in dividing all $81$ possible $2\times2$ matrices with elements $1, \omega$ and $\omega^2$ into the following $9$ LFP equivalence classes:


\subsection*{Class 0}
\noindent
\makeatletter\Hy@raisedlink{\hypertarget{d_3class0}}\makeatother
Singular Values: $\vec{s}= \left(1.0,\,0.0,\,0.0\right) $

\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ 0}}\makeatother : $f(x,y)=  0$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 0 & 0 \\
0 & 0 & 0
\end{array}\right)
$$

\subsection*{Class 1}
\noindent
\makeatletter\Hy@raisedlink{\hypertarget{d_3class1}}\makeatother
Singular Values: $\vec{s}= \left(0.90506,\,0.42527,\,0.0\right) $

\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ x^{2} y^{2} + x^{2} y + x y^{2} + x y}}\makeatother : $f(x,y)=  x^{2} y^{2} + x^{2} y + x y^{2} + x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 1 & 0 \\
0 & 0 & 0
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ x^{2} y^{2} + 2  x^{2} y + x y^{2} + 2  x y}}\makeatother : $f(x,y)=  x^{2} y^{2} + 2 \, x^{2} y + x y^{2} + 2 \, x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 0 & 1 \\
0 & 0 & 0
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ x^{2} y^{2} + x^{2} y + 2  x y^{2} + 2  x y}}\makeatother : $f(x,y)=  x^{2} y^{2} + x^{2} y + 2 \, x y^{2} + 2 \, x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 0 & 0 \\
0 & 1 & 0
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ x^{2} y^{2} + 2  x^{2} y + 2  x y^{2} + x y}}\makeatother : $f(x,y)=  x^{2} y^{2} + 2 \, x^{2} y + 2 \, x y^{2} + x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 0 & 0 \\
0 & 0 & 1
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ x^{2} y^{2} + x y^{2}}}\makeatother : $f(x,y)=  x^{2} y^{2} + x y^{2}$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 2 & 2 \\
0 & 0 & 0
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ x^{2} y^{2} + x^{2} y}}\makeatother : $f(x,y)=  x^{2} y^{2} + x^{2} y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 2 & 0 \\
0 & 2 & 0
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ x^{2} y^{2} + 2  x^{2} y}}\makeatother : $f(x,y)=  x^{2} y^{2} + 2 \, x^{2} y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 0 & 2 \\
0 & 0 & 2
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ x^{2} y^{2} + 2  x y^{2}}}\makeatother : $f(x,y)=  x^{2} y^{2} + 2 \, x y^{2}$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 0 & 0 \\
0 & 2 & 2
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ x^{2} y^{2}}}\makeatother : $f(x,y)=  x^{2} y^{2}$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 1 & 1 \\
0 & 1 & 1
\end{array}\right)
$$

\subsection*{Class 2}
\noindent
\makeatletter\Hy@raisedlink{\hypertarget{d_3class2}}\makeatother
Singular Values: $\vec{s}= \left(0.90506,\,0.42527,\,0.0\right) $

\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ 2  x^{2} y^{2} + 2  x^{2} y + 2  x y^{2} + 2  x y}}\makeatother : $f(x,y)=  2 \, x^{2} y^{2} + 2 \, x^{2} y + 2 \, x y^{2} + 2 \, x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 2 & 0 \\
0 & 0 & 0
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ 2  x^{2} y^{2} + x^{2} y + 2  x y^{2} + x y}}\makeatother : $f(x,y)=  2 \, x^{2} y^{2} + x^{2} y + 2 \, x y^{2} + x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 0 & 2 \\
0 & 0 & 0
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ 2  x^{2} y^{2} + 2  x^{2} y + x y^{2} + x y}}\makeatother : $f(x,y)=  2 \, x^{2} y^{2} + 2 \, x^{2} y + x y^{2} + x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 0 & 0 \\
0 & 2 & 0
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ 2  x^{2} y^{2} + x^{2} y + x y^{2} + 2  x y}}\makeatother : $f(x,y)=  2 \, x^{2} y^{2} + x^{2} y + x y^{2} + 2 \, x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 0 & 0 \\
0 & 0 & 2
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ 2  x^{2} y^{2} + 2  x y^{2}}}\makeatother : $f(x,y)=  2 \, x^{2} y^{2} + 2 \, x y^{2}$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 1 & 1 \\
0 & 0 & 0
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ 2  x^{2} y^{2} + 2  x^{2} y}}\makeatother : $f(x,y)=  2 \, x^{2} y^{2} + 2 \, x^{2} y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 1 & 0 \\
0 & 1 & 0
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ 2  x^{2} y^{2} + x^{2} y}}\makeatother : $f(x,y)=  2 \, x^{2} y^{2} + x^{2} y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 0 & 1 \\
0 & 0 & 1
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ 2  x^{2} y^{2} + x y^{2}}}\makeatother : $f(x,y)=  2 \, x^{2} y^{2} + x y^{2}$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 0 & 0 \\
0 & 1 & 1
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ 2  x^{2} y^{2}}}\makeatother : $f(x,y)=  2 \, x^{2} y^{2}$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 2 & 2 \\
0 & 2 & 2
\end{array}\right)
$$

\subsection*{Class 3}
\noindent
\makeatletter\Hy@raisedlink{\hypertarget{d_3class3}}\makeatother
Singular Values: $\vec{s}= \left(0.8165,\,0.57735,\,0.0\right) $

\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ 2  x y^{2}}}\makeatother : $f(x,y)=  2 \, x y^{2}$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 2 & 2 \\
0 & 1 & 1
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ x y^{2}}}\makeatother : $f(x,y)=  x y^{2}$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 1 & 1 \\
0 & 2 & 2
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ x y^{2} + x y}}\makeatother : $f(x,y)=  x y^{2} + x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 2 & 0 \\
0 & 1 & 0
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ 2  x y^{2} + 2  x y}}\makeatother : $f(x,y)=  2 \, x y^{2} + 2 \, x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 1 & 0 \\
0 & 2 & 0
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ x y^{2} + 2  x y}}\makeatother : $f(x,y)=  x y^{2} + 2 \, x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 0 & 2 \\
0 & 0 & 1
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ 2  x y^{2} + x y}}\makeatother : $f(x,y)=  2 \, x y^{2} + x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 0 & 1 \\
0 & 0 & 2
\end{array}\right)
$$

\subsection*{Class 4}
\noindent
\makeatletter\Hy@raisedlink{\hypertarget{d_3class4}}\makeatother
Singular Values: $\vec{s}= \left(0.8165,\,0.57735,\,0.0\right) $

\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ 2  x^{2} y}}\makeatother : $f(x,y)=  2 \, x^{2} y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 2 & 1 \\
0 & 2 & 1
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ x^{2} y}}\makeatother : $f(x,y)=  x^{2} y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 1 & 2 \\
0 & 1 & 2
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ 2  x^{2} y + x y}}\makeatother : $f(x,y)=  2 \, x^{2} y + x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 0 & 0 \\
0 & 1 & 2
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ x^{2} y + 2  x y}}\makeatother : $f(x,y)=  x^{2} y + 2 \, x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 0 & 0 \\
0 & 2 & 1
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ 2  x^{2} y + 2  x y}}\makeatother : $f(x,y)=  2 \, x^{2} y + 2 \, x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 1 & 2 \\
0 & 0 & 0
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ x^{2} y + x y}}\makeatother : $f(x,y)=  x^{2} y + x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 2 & 1 \\
0 & 0 & 0
\end{array}\right)
$$

\subsection*{Class 5}
\noindent
\makeatletter\Hy@raisedlink{\hypertarget{d_3class5}}\makeatother
Singular Values: $\vec{s}= \left(0.77814,\,0.57735,\,0.24732\right) $

\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ 2  x^{2} y^{2} + 2  x y}}\makeatother : $f(x,y)=  2 \, x^{2} y^{2} + 2 \, x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 1 & 0 \\
0 & 0 & 1
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ 2  x^{2} y^{2} + x y}}\makeatother : $f(x,y)=  2 \, x^{2} y^{2} + x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 0 & 1 \\
0 & 1 & 0
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ 2  x^{2} y^{2} + 2  x^{2} y + 2  x y}}\makeatother : $f(x,y)=  2 \, x^{2} y^{2} + 2 \, x^{2} y + 2 \, x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 0 & 1 \\
0 & 2 & 2
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ 2  x^{2} y^{2} + x^{2} y + x y}}\makeatother : $f(x,y)=  2 \, x^{2} y^{2} + x^{2} y + x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 1 & 0 \\
0 & 2 & 2
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ 2  x^{2} y^{2} + x^{2} y + 2  x y}}\makeatother : $f(x,y)=  2 \, x^{2} y^{2} + x^{2} y + 2 \, x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 2 & 2 \\
0 & 1 & 0
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ 2  x^{2} y^{2} + 2  x^{2} y + x y}}\makeatother : $f(x,y)=  2 \, x^{2} y^{2} + 2 \, x^{2} y + x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 2 & 2 \\
0 & 0 & 1
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ 2  x^{2} y^{2} + 2  x y^{2} + 2  x y}}\makeatother : $f(x,y)=  2 \, x^{2} y^{2} + 2 \, x y^{2} + 2 \, x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 0 & 2 \\
0 & 1 & 2
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ 2  x^{2} y^{2} + x y^{2} + x y}}\makeatother : $f(x,y)=  2 \, x^{2} y^{2} + x y^{2} + x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 1 & 2 \\
0 & 0 & 2
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ 2  x^{2} y^{2} + 2  x y^{2} + x y}}\makeatother : $f(x,y)=  2 \, x^{2} y^{2} + 2 \, x y^{2} + x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 2 & 0 \\
0 & 2 & 1
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ 2  x^{2} y^{2} + x y^{2} + 2  x y}}\makeatother : $f(x,y)=  2 \, x^{2} y^{2} + x y^{2} + 2 \, x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 2 & 1 \\
0 & 2 & 0
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ 2  x^{2} y^{2} + x^{2} y + x y^{2} + x y}}\makeatother : $f(x,y)=  2 \, x^{2} y^{2} + x^{2} y + x y^{2} + x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 2 & 1 \\
0 & 1 & 1
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ 2  x^{2} y^{2} + 2  x^{2} y + x y^{2} + 2  x y}}\makeatother : $f(x,y)=  2 \, x^{2} y^{2} + 2 \, x^{2} y + x y^{2} + 2 \, x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 1 & 2 \\
0 & 1 & 1
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ 2  x^{2} y^{2} + x^{2} y + 2  x y^{2} + 2  x y}}\makeatother : $f(x,y)=  2 \, x^{2} y^{2} + x^{2} y + 2 \, x y^{2} + 2 \, x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 1 & 1 \\
0 & 2 & 1
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ 2  x^{2} y^{2} + 2  x^{2} y + 2  x y^{2} + x y}}\makeatother : $f(x,y)=  2 \, x^{2} y^{2} + 2 \, x^{2} y + 2 \, x y^{2} + x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 1 & 1 \\
0 & 1 & 2
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ 2  x^{2} y^{2} + 2  x^{2} y + x y^{2}}}\makeatother : $f(x,y)=  2 \, x^{2} y^{2} + 2 \, x^{2} y + x y^{2}$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 2 & 1 \\
0 & 0 & 2
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ 2  x^{2} y^{2} + x^{2} y + 2  x y^{2}}}\makeatother : $f(x,y)=  2 \, x^{2} y^{2} + x^{2} y + 2 \, x y^{2}$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 2 & 0 \\
0 & 1 & 2
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ 2  x^{2} y^{2} + 2  x^{2} y + 2  x y^{2}}}\makeatother : $f(x,y)=  2 \, x^{2} y^{2} + 2 \, x^{2} y + 2 \, x y^{2}$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 0 & 2 \\
0 & 2 & 1
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ 2  x^{2} y^{2} + x^{2} y + x y^{2}}}\makeatother : $f(x,y)=  2 \, x^{2} y^{2} + x^{2} y + x y^{2}$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 1 & 2 \\
0 & 2 & 0
\end{array}\right)
$$

\subsection*{Class 6}
\noindent
\makeatletter\Hy@raisedlink{\hypertarget{d_3class6}}\makeatother
Singular Values: $\vec{s}= \left(0.77814,\,0.57735,\,0.24732\right) $

\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ x^{2} y^{2} + x y}}\makeatother : $f(x,y)=  x^{2} y^{2} + x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 2 & 0 \\
0 & 0 & 2
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ x^{2} y^{2} + 2  x y}}\makeatother : $f(x,y)=  x^{2} y^{2} + 2 \, x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 0 & 2 \\
0 & 2 & 0
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ x^{2} y^{2} + x^{2} y + x y}}\makeatother : $f(x,y)=  x^{2} y^{2} + x^{2} y + x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 0 & 2 \\
0 & 1 & 1
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ x^{2} y^{2} + 2  x^{2} y + 2  x y}}\makeatother : $f(x,y)=  x^{2} y^{2} + 2 \, x^{2} y + 2 \, x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 2 & 0 \\
0 & 1 & 1
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ x^{2} y^{2} + 2  x^{2} y + x y}}\makeatother : $f(x,y)=  x^{2} y^{2} + 2 \, x^{2} y + x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 1 & 1 \\
0 & 2 & 0
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ x^{2} y^{2} + x^{2} y + 2  x y}}\makeatother : $f(x,y)=  x^{2} y^{2} + x^{2} y + 2 \, x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 1 & 1 \\
0 & 0 & 2
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ x^{2} y^{2} + x y^{2} + x y}}\makeatother : $f(x,y)=  x^{2} y^{2} + x y^{2} + x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 0 & 1 \\
0 & 2 & 1
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ x^{2} y^{2} + 2  x y^{2} + 2  x y}}\makeatother : $f(x,y)=  x^{2} y^{2} + 2 \, x y^{2} + 2 \, x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 2 & 1 \\
0 & 0 & 1
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ x^{2} y^{2} + x y^{2} + 2  x y}}\makeatother : $f(x,y)=  x^{2} y^{2} + x y^{2} + 2 \, x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 1 & 0 \\
0 & 1 & 2
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ x^{2} y^{2} + 2  x y^{2} + x y}}\makeatother : $f(x,y)=  x^{2} y^{2} + 2 \, x y^{2} + x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 1 & 2 \\
0 & 1 & 0
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ x^{2} y^{2} + 2  x^{2} y + 2  x y^{2} + 2  x y}}\makeatother : $f(x,y)=  x^{2} y^{2} + 2 \, x^{2} y + 2 \, x y^{2} + 2 \, x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 1 & 2 \\
0 & 2 & 2
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ x^{2} y^{2} + x^{2} y + 2  x y^{2} + x y}}\makeatother : $f(x,y)=  x^{2} y^{2} + x^{2} y + 2 \, x y^{2} + x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 2 & 1 \\
0 & 2 & 2
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ x^{2} y^{2} + 2  x^{2} y + x y^{2} + x y}}\makeatother : $f(x,y)=  x^{2} y^{2} + 2 \, x^{2} y + x y^{2} + x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 2 & 2 \\
0 & 1 & 2
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ x^{2} y^{2} + x^{2} y + x y^{2} + 2  x y}}\makeatother : $f(x,y)=  x^{2} y^{2} + x^{2} y + x y^{2} + 2 \, x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 2 & 2 \\
0 & 2 & 1
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ x^{2} y^{2} + x^{2} y + 2  x y^{2}}}\makeatother : $f(x,y)=  x^{2} y^{2} + x^{2} y + 2 \, x y^{2}$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 1 & 2 \\
0 & 0 & 1
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ x^{2} y^{2} + 2  x^{2} y + x y^{2}}}\makeatother : $f(x,y)=  x^{2} y^{2} + 2 \, x^{2} y + x y^{2}$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 1 & 0 \\
0 & 2 & 1
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ x^{2} y^{2} + x^{2} y + x y^{2}}}\makeatother : $f(x,y)=  x^{2} y^{2} + x^{2} y + x y^{2}$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 0 & 1 \\
0 & 1 & 2
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ x^{2} y^{2} + 2  x^{2} y + 2  x y^{2}}}\makeatother : $f(x,y)=  x^{2} y^{2} + 2 \, x^{2} y + 2 \, x y^{2}$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 2 & 1 \\
0 & 1 & 0
\end{array}\right)
$$

\subsection*{Class 7}
\noindent
\makeatletter\Hy@raisedlink{\hypertarget{d_3class7}}\makeatother
Singular Values: $\vec{s}= \left(0.84403,\,0.4491,\,0.29313\right) $

\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ 2  x^{2} y + 2  x y^{2}}}\makeatother : $f(x,y)=  2 \, x^{2} y + 2 \, x y^{2}$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 1 & 0 \\
0 & 0 & 2
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ x^{2} y + x y^{2}}}\makeatother : $f(x,y)=  x^{2} y + x y^{2}$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 2 & 0 \\
0 & 0 & 1
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ x^{2} y + 2  x y^{2}}}\makeatother : $f(x,y)=  x^{2} y + 2 \, x y^{2}$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 0 & 1 \\
0 & 2 & 0
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ 2  x^{2} y + x y^{2}}}\makeatother : $f(x,y)=  2 \, x^{2} y + x y^{2}$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 0 & 2 \\
0 & 1 & 0
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ x^{2} y + x y^{2} + 2  x y}}\makeatother : $f(x,y)=  x^{2} y + x y^{2} + 2 \, x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 1 & 1 \\
0 & 1 & 0
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ 2  x^{2} y + x y^{2} + x y}}\makeatother : $f(x,y)=  2 \, x^{2} y + x y^{2} + x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 1 & 1 \\
0 & 0 & 1
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ x^{2} y + 2  x y^{2} + x y}}\makeatother : $f(x,y)=  x^{2} y + 2 \, x y^{2} + x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 1 & 0 \\
0 & 1 & 1
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ 2  x^{2} y + 2  x y^{2} + 2  x y}}\makeatother : $f(x,y)=  2 \, x^{2} y + 2 \, x y^{2} + 2 \, x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 0 & 1 \\
0 & 1 & 1
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ 2  x^{2} y + 2  x y^{2} + x y}}\makeatother : $f(x,y)=  2 \, x^{2} y + 2 \, x y^{2} + x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 2 & 2 \\
0 & 2 & 0
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ x^{2} y + 2  x y^{2} + 2  x y}}\makeatother : $f(x,y)=  x^{2} y + 2 \, x y^{2} + 2 \, x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 2 & 2 \\
0 & 0 & 2
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ 2  x^{2} y + x y^{2} + 2  x y}}\makeatother : $f(x,y)=  2 \, x^{2} y + x y^{2} + 2 \, x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 2 & 0 \\
0 & 2 & 2
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ x^{2} y + x y^{2} + x y}}\makeatother : $f(x,y)=  x^{2} y + x y^{2} + x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 0 & 2 \\
0 & 2 & 2
\end{array}\right)
$$

\subsection*{Class 8}
\noindent
\makeatletter\Hy@raisedlink{\hypertarget{d_3class8}}\makeatother
Singular Values: $\vec{s}= \left(0.57735,\,0.57735,\,0.57735\right) $

\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ 2  x y}}\makeatother : $f(x,y)=  2 \, x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 2 & 1 \\
0 & 1 & 2
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{d3_ x y}}\makeatother : $f(x,y)=  x y$
$$
M_f = 
\left(\begin{array}{rrr}
0 & 0 & 0 \\
0 & 1 & 2 \\
0 & 2 & 1
\end{array}\right)
$$



\section{LFP and LU classes of bipartite ququarts}\label{AP:ququartClasses}

\begin{longtable}{ |c|c|l| }
\caption{The full classification of the equivalences of bipartite \emph{TEH} states und LU and LFP operations in dimension $4$. 
The horizontal lines indicate different LFP classes while the singular values identify different LU classes. \label{table:d4classes}}
\\
\hline
Schmidt Rank & Singular Values & Polynomial \\
\hline
\endfirsthead

\hline
Schmidt Rank & Singular Values & Polynomial \\
\hline
\endhead
\pagebreak[2]
\multirow{1}{4em}{$1$}&\multirow{1}{*}{\hyperlink{class0}{$\left(1.0,\,0.0,\,0.0,\,0.0\right)$}}&\hyperlink{0}{$f(x,y)= 0$}\Tstrut
\\*
\hline
\pagebreak[2]
\multirow{2}{4em}{$2$}&\multirow{2}{*}{\hyperlink{class1}{$\left(0.92388,\,0.38268,\,0.0,\,0.0\right)$}}&\hyperlink{x^{2} y + x y^{2} + x y}{$f(x,y)= x^{2} y + x y^{2} + x y$}\Tstrut
\\*
\pagebreak[2]
&&\hyperlink{x^{2} y + x y^{2} + 3  x y}{$f(x,y)= x^{2} y + x y^{2} + 3 \, x y$}
\\*
\hline
\pagebreak[2]
\multirow{4}{4em}{$2$}&\multirow{4}{*}{\hyperlink{class2}{$\left(0.86603,\,0.5,\,0.0,\,0.0\right)$}}&\hyperlink{x y^{3} + x y^{2}}{$f(x,y)= x y^{3} + x y^{2}$}\Tstrut
\\*
\pagebreak[2]
&&\hyperlink{x y^{3} + x y}{$f(x,y)= x y^{3} + x y$}
\\*
\pagebreak[2]
&&\hyperlink{x y^{3} + x y^{2} + 2  x y}{$f(x,y)= x y^{3} + x y^{2} + 2 \, x y$}
\\*
\pagebreak[2]
&&\hyperlink{x y^{3} + 3  x y}{$f(x,y)= x y^{3} + 3 \, x y$}
\\*
\hline
\pagebreak[2]
\multirow{4}{4em}{$2$}&\multirow{4}{*}{\hyperlink{class3}{$\left(0.86603,\,0.5,\,0.0,\,0.0\right)$}}&\hyperlink{x^{3} y + x^{2} y}{$f(x,y)= x^{3} y + x^{2} y$}\Tstrut
\\*
\pagebreak[2]
&&\hyperlink{x^{3} y + x y}{$f(x,y)= x^{3} y + x y$}
\\*
\pagebreak[2]
&&\hyperlink{x^{3} y + x^{2} y + 2  x y}{$f(x,y)= x^{3} y + x^{2} y + 2 \, x y$}
\\*
\pagebreak[2]
&&\hyperlink{x^{3} y + 3  x y}{$f(x,y)= x^{3} y + 3 \, x y$}
\\*
\hline
\pagebreak[2]
\multirow{4}{4em}{$2$}&\multirow{4}{*}{\hyperlink{class4}{$\left(0.86603,\,0.5,\,0.0,\,0.0\right)$}}&\hyperlink{x y^{3} + x^{2} y + x y^{2}}{$f(x,y)= x y^{3} + x^{2} y + x y^{2}$}\Tstrut
\\*
\pagebreak[2]
&&\hyperlink{x y^{3} + x^{2} y + x y}{$f(x,y)= x y^{3} + x^{2} y + x y$}
\\*
\pagebreak[2]
&&\hyperlink{x y^{3} + x^{2} y + x y^{2} + 2  x y}{$f(x,y)= x y^{3} + x^{2} y + x y^{2} + 2 \, x y$}
\\*
\pagebreak[2]
&&\hyperlink{x y^{3} + x^{2} y + 3  x y}{$f(x,y)= x y^{3} + x^{2} y + 3 \, x y$}
\\*
\hline
\pagebreak[2]
\multirow{4}{4em}{$2$}&\multirow{4}{*}{\hyperlink{class5}{$\left(0.86603,\,0.5,\,0.0,\,0.0\right)$}}&\hyperlink{x^{3} y + x^{2} y + x y^{2}}{$f(x,y)= x^{3} y + x^{2} y + x y^{2}$}\Tstrut
\\*
\pagebreak[2]
&&\hyperlink{x^{3} y + x y^{2} + x y}{$f(x,y)= x^{3} y + x y^{2} + x y$}
\\*
\pagebreak[2]
&&\hyperlink{x^{3} y + x^{2} y + x y^{2} + 2  x y}{$f(x,y)= x^{3} y + x^{2} y + x y^{2} + 2 \, x y$}
\\*
\pagebreak[2]
&&\hyperlink{x^{3} y + x y^{2} + 3  x y}{$f(x,y)= x^{3} y + x y^{2} + 3 \, x y$}
\\*
\hline
\pagebreak[4]
\multirow{5}{4em}{$2$}&\multirow{5}{*}{\hyperlink{class6}{$\left(0.70711,\,0.70711,\,0.0,\,0.0\right)$}}&\hyperlink{x^{2} y + x y}{$f(x,y)= x^{2} y + x y$}\Tstrut
\\*
\pagebreak[2]
&&\hyperlink{x y^{2} + x y}{$f(x,y)= x y^{2} + x y$}
\\*
\pagebreak[2]
&&\hyperlink{2  x y}{$f(x,y)= 2 \, x y$}
\\*
\pagebreak[2]
&&\hyperlink{x^{2} y + 3  x y}{$f(x,y)= x^{2} y + 3 \, x y$}
\\*
\pagebreak[2]
&&\hyperlink{x y^{2} + 3  x y}{$f(x,y)= x y^{2} + 3 \, x y$}
\\*
\hline
\pagebreak[2]
\multirow{2}{4em}{$2$}&\multirow{2}{*}{\hyperlink{class7}{$\left(0.70711,\,0.70711,\,0.0,\,0.0\right)$}}&\hyperlink{x y^{2}}{$f(x,y)= x y^{2}$}\Tstrut
\\*
\pagebreak[2]
&&\hyperlink{x y^{2} + 2  x y}{$f(x,y)= x y^{2} + 2 \, x y$}
\\*
\hline
\pagebreak[2]
\multirow{2}{4em}{$2$}&\multirow{2}{*}{\hyperlink{class8}{$\left(0.70711,\,0.70711,\,0.0,\,0.0\right)$}}&\hyperlink{x^{2} y}{$f(x,y)= x^{2} y$}\Tstrut
\\*
\pagebreak[2]
&&\hyperlink{x^{2} y + 2  x y}{$f(x,y)= x^{2} y + 2 \, x y$}
\\*
\hline
\pagebreak[2]
\multirow{8}{4em}{$3$}&\multirow{8}{*}{\hyperlink{class9}{$\left(0.80902,\,0.5,\,0.30902,\,0.0\right)$}}&\hyperlink{x^{3} y + x y^{3}}{$f(x,y)= x^{3} y + x y^{3}$}\Tstrut
\\*
\pagebreak[2]
&&\hyperlink{x^{3} y + x y^{3} + x^{2} y + x y^{2}}{$f(x,y)= x^{3} y + x y^{3} + x^{2} y + x y^{2}$}
\\*
\pagebreak[2]
&&\hyperlink{x^{3} y + x y^{3} + x^{2} y + x y}{$f(x,y)= x^{3} y + x y^{3} + x^{2} y + x y$}
\\*
\pagebreak[2]
&&\hyperlink{x^{3} y + x y^{3} + x y^{2} + x y}{$f(x,y)= x^{3} y + x y^{3} + x y^{2} + x y$}
\\*
\pagebreak[2]
&&\hyperlink{x^{3} y + x y^{3} + 2  x y}{$f(x,y)= x^{3} y + x y^{3} + 2 \, x y$}
\\*
\pagebreak[2]
&&\hyperlink{x^{3} y + x y^{3} + x^{2} y + x y^{2} + 2  x y}{$f(x,y)= x^{3} y + x y^{3} + x^{2} y + x y^{2} + 2 \, x y$}
\\*
\pagebreak[2]
&&\hyperlink{x^{3} y + x y^{3} + x^{2} y + 3  x y}{$f(x,y)= x^{3} y + x y^{3} + x^{2} y + 3 \, x y$}
\\*
\pagebreak[2]
&&\hyperlink{x^{3} y + x y^{3} + x y^{2} + 3  x y}{$f(x,y)= x^{3} y + x y^{3} + x y^{2} + 3 \, x y$}
\\*
\hline
\pagebreak[2]
\multirow{8}{4em}{$3$}&\multirow{8}{*}{\hyperlink{class10}{$\left(0.80902,\,0.5,\,0.30902,\,0.0\right)$}}&\hyperlink{x^{3} y + x y^{3} + x^{2} y}{$f(x,y)= x^{3} y + x y^{3} + x^{2} y$}\Tstrut
\\*
\pagebreak[2]
&&\hyperlink{x^{3} y + x y^{3} + x y^{2}}{$f(x,y)= x^{3} y + x y^{3} + x y^{2}$}
\\*
\pagebreak[2]
&&\hyperlink{x^{3} y + x y^{3} + x y}{$f(x,y)= x^{3} y + x y^{3} + x y$}
\\*
\pagebreak[2]
&&\hyperlink{x^{3} y + x y^{3} + x^{2} y + x y^{2} + x y}{$f(x,y)= x^{3} y + x y^{3} + x^{2} y + x y^{2} + x y$}
\\*
\pagebreak[2]
&&\hyperlink{x^{3} y + x y^{3} + x^{2} y + 2  x y}{$f(x,y)= x^{3} y + x y^{3} + x^{2} y + 2 \, x y$}
\\*
\pagebreak[2]
&&\hyperlink{x^{3} y + x y^{3} + x y^{2} + 2  x y}{$f(x,y)= x^{3} y + x y^{3} + x y^{2} + 2 \, x y$}
\\*
\pagebreak[2]
&&\hyperlink{x^{3} y + x y^{3} + 3  x y}{$f(x,y)= x^{3} y + x y^{3} + 3 \, x y$}
\\*
\pagebreak[2]
&&\hyperlink{x^{3} y + x y^{3} + x^{2} y + x y^{2} + 3  x y}{$f(x,y)= x^{3} y + x y^{3} + x^{2} y + x y^{2} + 3 \, x y$}
\\*
\hline
\pagebreak[2]
\multirow{4}{4em}{$3$}&\multirow{4}{*}{\hyperlink{class11}{$\left(0.70711,\,0.5,\,0.5,\,0.0\right)$}}&\hyperlink{x y^{3} + x^{2} y}{$f(x,y)= x y^{3} + x^{2} y$}\Tstrut
\\*
\pagebreak[2]
&&\hyperlink{x y^{3} + x^{2} y + x y^{2} + x y}{$f(x,y)= x y^{3} + x^{2} y + x y^{2} + x y$}
\\*
\pagebreak[2]
&&\hyperlink{x y^{3} + x^{2} y + 2  x y}{$f(x,y)= x y^{3} + x^{2} y + 2 \, x y$}
\\*
\pagebreak[2]
&&\hyperlink{x y^{3} + x^{2} y + x y^{2} + 3  x y}{$f(x,y)= x y^{3} + x^{2} y + x y^{2} + 3 \, x y$}
\\*
\hline
\pagebreak[2]
\multirow{4}{4em}{$3$}&\multirow{4}{*}{\hyperlink{class12}{$\left(0.70711,\,0.5,\,0.5,\,0.0\right)$}}&\hyperlink{x y^{3}}{$f(x,y)= x y^{3}$}\Tstrut
\\*
\pagebreak[2]
&&\hyperlink{x y^{3} + x y^{2} + x y}{$f(x,y)= x y^{3} + x y^{2} + x y$}
\\*
\pagebreak[2]
&&\hyperlink{x y^{3} + 2  x y}{$f(x,y)= x y^{3} + 2 \, x y$}
\\*
\pagebreak[2]
&&\hyperlink{x y^{3} + x y^{2} + 3  x y}{$f(x,y)= x y^{3} + x y^{2} + 3 \, x y$}
\\*
\hline
\pagebreak[2]
\multirow{4}{4em}{$3$}&\multirow{4}{*}{\hyperlink{class13}{$\left(0.70711,\,0.5,\,0.5,\,0.0\right)$}}&\hyperlink{x^{3} y + x y^{2}}{$f(x,y)= x^{3} y + x y^{2}$}\Tstrut
\\*
\pagebreak[2]
&&\hyperlink{x^{3} y + x^{2} y + x y^{2} + x y}{$f(x,y)= x^{3} y + x^{2} y + x y^{2} + x y$}
\\*
\pagebreak[2]
&&\hyperlink{x^{3} y + x y^{2} + 2  x y}{$f(x,y)= x^{3} y + x y^{2} + 2 \, x y$}
\\*
\pagebreak[2]
&&\hyperlink{x^{3} y + x^{2} y + x y^{2} + 3  x y}{$f(x,y)= x^{3} y + x^{2} y + x y^{2} + 3 \, x y$}
\\*
\hline
\pagebreak[2]
\multirow{4}{4em}{$3$}&\multirow{4}{*}{\hyperlink{class14}{$\left(0.70711,\,0.5,\,0.5,\,0.0\right)$}}&\hyperlink{x^{3} y}{$f(x,y)= x^{3} y$}\Tstrut
\\*
\pagebreak[2]
&&\hyperlink{x^{3} y + x^{2} y + x y}{$f(x,y)= x^{3} y + x^{2} y + x y$}
\\*
\pagebreak[2]
&&\hyperlink{x^{3} y + 2  x y}{$f(x,y)= x^{3} y + 2 \, x y$}
\\*
\pagebreak[2]
&&\hyperlink{x^{3} y + x^{2} y + 3  x y}{$f(x,y)= x^{3} y + x^{2} y + 3 \, x y$}
\\*
\hline
\pagebreak[2]
\multirow{2}{4em}{$4$}&\multirow{2}{*}{\hyperlink{class15}{$\left(0.5,\,0.5,\,0.5,\,0.5\right)$}}&\hyperlink{x^{2} y + x y^{2}}{$f(x,y)= x^{2} y + x y^{2}$}\Tstrut
\\*
\pagebreak[2]
&&\hyperlink{x^{2} y + x y^{2} + 2  x y}{$f(x,y)= x^{2} y + x y^{2} + 2 \, x y$}
\\*
\hline
\pagebreak[2]
\multirow{2}{4em}{$4$}&\multirow{2}{*}{\hyperlink{class16}{$\left(0.5,\,0.5,\,0.5,\,0.5\right)$}}&\hyperlink{x y}{$f(x,y)= x y$}\Tstrut
\\*
\pagebreak[2]
&&\hyperlink{3  x y}{$f(x,y)= 3 \, x y$}
\\*
\hline
\end{longtable}





\subsection*{Class 0}
\noindent
\makeatletter\Hy@raisedlink{\hypertarget{class0}}\makeatother
Singular Values: $\vec{s}= \left(1.0,\,0.0,\,0.0,\,0.0\right) $

\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{0}}\makeatother : $f(x,y)= 0$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0
\end{array}\right)
$$

\subsection*{Class 1}
\noindent
\makeatletter\Hy@raisedlink{\hypertarget{class1}}\makeatother
Singular Values: $\vec{s}= \left(0.92388,\,0.38268,\,0.0,\,0.0\right) $

\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x^{2} y + x y^{2} + x y}}\makeatother : $f(x,y)= x^{2} y + x y^{2} + x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 3 & 0 & 3 \\
0 & 0 & 0 & 0 \\
0 & 3 & 0 & 3
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x^{2} y + x y^{2} + 3  x y}}\makeatother : $f(x,y)= x^{2} y + x y^{2} + 3 \, x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 1 & 0 & 1 \\
0 & 0 & 0 & 0 \\
0 & 1 & 0 & 1
\end{array}\right)
$$

\subsection*{Class 2}
\noindent
\makeatletter\Hy@raisedlink{\hypertarget{class2}}\makeatother
Singular Values: $\vec{s}= \left(0.86603,\,0.5,\,0.0,\,0.0\right) $

\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x y^{3} + x y^{2}}}\makeatother : $f(x,y)= x y^{3} + x y^{2}$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 2 & 0 & 2 \\
0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x y^{3} + x y}}\makeatother : $f(x,y)= x y^{3} + x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 2 & 0 & 2 \\
0 & 2 & 0 & 2 \\
0 & 2 & 0 & 2
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x y^{3} + x y^{2} + 2  x y}}\makeatother : $f(x,y)= x y^{3} + x y^{2} + 2 \, x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 \\
0 & 2 & 0 & 2
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x y^{3} + 3  x y}}\makeatother : $f(x,y)= x y^{3} + 3 \, x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 \\
0 & 2 & 0 & 2 \\
0 & 0 & 0 & 0
\end{array}\right)
$$

\subsection*{Class 3}
\noindent
\makeatletter\Hy@raisedlink{\hypertarget{class3}}\makeatother
Singular Values: $\vec{s}= \left(0.86603,\,0.5,\,0.0,\,0.0\right) $

\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x^{3} y + x^{2} y}}\makeatother : $f(x,y)= x^{3} y + x^{2} y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 2 & 0 & 0 \\
0 & 0 & 0 & 0 \\
0 & 2 & 0 & 0
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x^{3} y + x y}}\makeatother : $f(x,y)= x^{3} y + x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 2 & 2 & 2 \\
0 & 0 & 0 & 0 \\
0 & 2 & 2 & 2
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x^{3} y + x^{2} y + 2  x y}}\makeatother : $f(x,y)= x^{3} y + x^{2} y + 2 \, x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 0 & 0 & 2 \\
0 & 0 & 0 & 0 \\
0 & 0 & 0 & 2
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x^{3} y + 3  x y}}\makeatother : $f(x,y)= x^{3} y + 3 \, x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 0 & 2 & 0 \\
0 & 0 & 0 & 0 \\
0 & 0 & 2 & 0
\end{array}\right)
$$

\subsection*{Class 4}
\noindent
\makeatletter\Hy@raisedlink{\hypertarget{class4}}\makeatother
Singular Values: $\vec{s}= \left(0.86603,\,0.5,\,0.0,\,0.0\right) $

\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x y^{3} + x^{2} y + x y^{2}}}\makeatother : $f(x,y)= x y^{3} + x^{2} y + x y^{2}$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 3 & 0 & 3 \\
0 & 2 & 0 & 2 \\
0 & 3 & 0 & 3
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x y^{3} + x^{2} y + x y}}\makeatother : $f(x,y)= x y^{3} + x^{2} y + x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 3 & 0 & 3 \\
0 & 0 & 0 & 0 \\
0 & 1 & 0 & 1
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x y^{3} + x^{2} y + x y^{2} + 2  x y}}\makeatother : $f(x,y)= x y^{3} + x^{2} y + x y^{2} + 2 \, x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 1 & 0 & 1 \\
0 & 2 & 0 & 2 \\
0 & 1 & 0 & 1
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x y^{3} + x^{2} y + 3  x y}}\makeatother : $f(x,y)= x y^{3} + x^{2} y + 3 \, x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 1 & 0 & 1 \\
0 & 0 & 0 & 0 \\
0 & 3 & 0 & 3
\end{array}\right)
$$

\subsection*{Class 5}
\noindent
\makeatletter\Hy@raisedlink{\hypertarget{class5}}\makeatother
Singular Values: $\vec{s}= \left(0.86603,\,0.5,\,0.0,\,0.0\right) $

\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x^{3} y + x^{2} y + x y^{2}}}\makeatother : $f(x,y)= x^{3} y + x^{2} y + x y^{2}$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 3 & 2 & 3 \\
0 & 0 & 0 & 0 \\
0 & 3 & 2 & 3
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x^{3} y + x y^{2} + x y}}\makeatother : $f(x,y)= x^{3} y + x y^{2} + x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 3 & 0 & 1 \\
0 & 0 & 0 & 0 \\
0 & 3 & 0 & 1
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x^{3} y + x^{2} y + x y^{2} + 2  x y}}\makeatother : $f(x,y)= x^{3} y + x^{2} y + x y^{2} + 2 \, x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 1 & 2 & 1 \\
0 & 0 & 0 & 0 \\
0 & 1 & 2 & 1
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x^{3} y + x y^{2} + 3  x y}}\makeatother : $f(x,y)= x^{3} y + x y^{2} + 3 \, x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 1 & 0 & 3 \\
0 & 0 & 0 & 0 \\
0 & 1 & 0 & 3
\end{array}\right)
$$

\subsection*{Class 6}
\noindent
\makeatletter\Hy@raisedlink{\hypertarget{class6}}\makeatother
Singular Values: $\vec{s}= \left(0.70711,\,0.70711,\,0.0,\,0.0\right) $

\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x^{2} y + x y}}\makeatother : $f(x,y)= x^{2} y + x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 2 & 2 & 0 \\
0 & 0 & 0 & 0 \\
0 & 2 & 2 & 0
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x y^{2} + x y}}\makeatother : $f(x,y)= x y^{2} + x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 2 & 0 & 2 \\
0 & 2 & 0 & 2 \\
0 & 0 & 0 & 0
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{2  x y}}\makeatother : $f(x,y)= 2 \, x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 2 & 0 & 2 \\
0 & 0 & 0 & 0 \\
0 & 2 & 0 & 2
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x^{2} y + 3  x y}}\makeatother : $f(x,y)= x^{2} y + 3 \, x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 0 & 2 & 2 \\
0 & 0 & 0 & 0 \\
0 & 0 & 2 & 2
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x y^{2} + 3  x y}}\makeatother : $f(x,y)= x y^{2} + 3 \, x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 \\
0 & 2 & 0 & 2 \\
0 & 2 & 0 & 2
\end{array}\right)
$$

\subsection*{Class 7}
\noindent
\makeatletter\Hy@raisedlink{\hypertarget{class7}}\makeatother
Singular Values: $\vec{s}= \left(0.70711,\,0.70711,\,0.0,\,0.0\right) $

\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x y^{2}}}\makeatother : $f(x,y)= x y^{2}$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 1 & 2 & 3 \\
0 & 0 & 0 & 0 \\
0 & 1 & 2 & 3
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x y^{2} + 2  x y}}\makeatother : $f(x,y)= x y^{2} + 2 \, x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 3 & 2 & 1 \\
0 & 0 & 0 & 0 \\
0 & 3 & 2 & 1
\end{array}\right)
$$

\subsection*{Class 8}
\noindent
\makeatletter\Hy@raisedlink{\hypertarget{class8}}\makeatother
Singular Values: $\vec{s}= \left(0.70711,\,0.70711,\,0.0,\,0.0\right) $

\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x^{2} y}}\makeatother : $f(x,y)= x^{2} y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 1 & 0 & 1 \\
0 & 2 & 0 & 2 \\
0 & 3 & 0 & 3
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x^{2} y + 2  x y}}\makeatother : $f(x,y)= x^{2} y + 2 \, x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 3 & 0 & 3 \\
0 & 2 & 0 & 2 \\
0 & 1 & 0 & 1
\end{array}\right)
$$

\subsection*{Class 9}
\noindent
\makeatletter\Hy@raisedlink{\hypertarget{class9}}\makeatother
Singular Values: $\vec{s}= \left(0.80902,\,0.5,\,0.30902,\,0.0\right) $

\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x^{3} y + x y^{3}}}\makeatother : $f(x,y)= x^{3} y + x y^{3}$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 2 & 2 & 2 \\
0 & 2 & 0 & 2 \\
0 & 2 & 2 & 2
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x^{3} y + x y^{3} + x^{2} y + x y^{2}}}\makeatother : $f(x,y)= x^{3} y + x y^{3} + x^{2} y + x y^{2}$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 0 & 0 & 2 \\
0 & 0 & 0 & 0 \\
0 & 2 & 0 & 0
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x^{3} y + x y^{3} + x^{2} y + x y}}\makeatother : $f(x,y)= x^{3} y + x y^{3} + x^{2} y + x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 0 & 0 & 2 \\
0 & 2 & 0 & 2 \\
0 & 0 & 0 & 2
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x^{3} y + x y^{3} + x y^{2} + x y}}\makeatother : $f(x,y)= x^{3} y + x y^{3} + x y^{2} + x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 0 & 2 & 0 \\
0 & 0 & 0 & 0 \\
0 & 2 & 2 & 2
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x^{3} y + x y^{3} + 2  x y}}\makeatother : $f(x,y)= x^{3} y + x y^{3} + 2 \, x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 0 & 2 & 0 \\
0 & 2 & 0 & 2 \\
0 & 0 & 2 & 0
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x^{3} y + x y^{3} + x^{2} y + x y^{2} + 2  x y}}\makeatother : $f(x,y)= x^{3} y + x y^{3} + x^{2} y + x y^{2} + 2 \, x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 2 & 0 & 0 \\
0 & 0 & 0 & 0 \\
0 & 0 & 0 & 2
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x^{3} y + x y^{3} + x^{2} y + 3  x y}}\makeatother : $f(x,y)= x^{3} y + x y^{3} + x^{2} y + 3 \, x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 2 & 0 & 0 \\
0 & 2 & 0 & 2 \\
0 & 2 & 0 & 0
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x^{3} y + x y^{3} + x y^{2} + 3  x y}}\makeatother : $f(x,y)= x^{3} y + x y^{3} + x y^{2} + 3 \, x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 2 & 2 & 2 \\
0 & 0 & 0 & 0 \\
0 & 0 & 2 & 0
\end{array}\right)
$$

\subsection*{Class 10}
\noindent
\makeatletter\Hy@raisedlink{\hypertarget{class10}}\makeatother
Singular Values: $\vec{s}= \left(0.80902,\,0.5,\,0.30902,\,0.0\right) $

\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x^{3} y + x y^{3} + x^{2} y}}\makeatother : $f(x,y)= x^{3} y + x y^{3} + x^{2} y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 3 & 2 & 3 \\
0 & 0 & 0 & 0 \\
0 & 1 & 2 & 1
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x^{3} y + x y^{3} + x y^{2}}}\makeatother : $f(x,y)= x^{3} y + x y^{3} + x y^{2}$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 3 & 0 & 1 \\
0 & 2 & 0 & 2 \\
0 & 3 & 0 & 1
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x^{3} y + x y^{3} + x y}}\makeatother : $f(x,y)= x^{3} y + x y^{3} + x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 3 & 0 & 1 \\
0 & 0 & 0 & 0 \\
0 & 1 & 0 & 3
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x^{3} y + x y^{3} + x^{2} y + x y^{2} + x y}}\makeatother : $f(x,y)= x^{3} y + x y^{3} + x^{2} y + x y^{2} + x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 1 & 2 & 1 \\
0 & 2 & 0 & 2 \\
0 & 1 & 2 & 1
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x^{3} y + x y^{3} + x^{2} y + 2  x y}}\makeatother : $f(x,y)= x^{3} y + x y^{3} + x^{2} y + 2 \, x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 1 & 2 & 1 \\
0 & 0 & 0 & 0 \\
0 & 3 & 2 & 3
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x^{3} y + x y^{3} + x y^{2} + 2  x y}}\makeatother : $f(x,y)= x^{3} y + x y^{3} + x y^{2} + 2 \, x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 1 & 0 & 3 \\
0 & 2 & 0 & 2 \\
0 & 1 & 0 & 3
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x^{3} y + x y^{3} + 3  x y}}\makeatother : $f(x,y)= x^{3} y + x y^{3} + 3 \, x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 1 & 0 & 3 \\
0 & 0 & 0 & 0 \\
0 & 3 & 0 & 1
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x^{3} y + x y^{3} + x^{2} y + x y^{2} + 3  x y}}\makeatother : $f(x,y)= x^{3} y + x y^{3} + x^{2} y + x y^{2} + 3 \, x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 3 & 2 & 3 \\
0 & 2 & 0 & 2 \\
0 & 3 & 2 & 3
\end{array}\right)
$$

\subsection*{Class 11}
\noindent
\makeatletter\Hy@raisedlink{\hypertarget{class11}}\makeatother
Singular Values: $\vec{s}= \left(0.70711,\,0.5,\,0.5,\,0.0\right) $

\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x y^{3} + x^{2} y}}\makeatother : $f(x,y)= x y^{3} + x^{2} y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 2 & 2 & 0 \\
0 & 2 & 0 & 2 \\
0 & 2 & 2 & 0
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x y^{3} + x^{2} y + x y^{2} + x y}}\makeatother : $f(x,y)= x y^{3} + x^{2} y + x y^{2} + x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 0 & 2 & 2 \\
0 & 0 & 0 & 0 \\
0 & 2 & 2 & 0
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x y^{3} + x^{2} y + 2  x y}}\makeatother : $f(x,y)= x y^{3} + x^{2} y + 2 \, x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 0 & 2 & 2 \\
0 & 2 & 0 & 2 \\
0 & 0 & 2 & 2
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x y^{3} + x^{2} y + x y^{2} + 3  x y}}\makeatother : $f(x,y)= x y^{3} + x^{2} y + x y^{2} + 3 \, x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 2 & 2 & 0 \\
0 & 0 & 0 & 0 \\
0 & 0 & 2 & 2
\end{array}\right)
$$

\subsection*{Class 12}
\noindent
\makeatletter\Hy@raisedlink{\hypertarget{class12}}\makeatother
Singular Values: $\vec{s}= \left(0.70711,\,0.5,\,0.5,\,0.0\right) $

\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x y^{3}}}\makeatother : $f(x,y)= x y^{3}$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 1 & 2 & 3 \\
0 & 0 & 0 & 0 \\
0 & 3 & 2 & 1
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x y^{3} + x y^{2} + x y}}\makeatother : $f(x,y)= x y^{3} + x y^{2} + x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 3 & 2 & 1 \\
0 & 2 & 0 & 2 \\
0 & 3 & 2 & 1
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x y^{3} + 2  x y}}\makeatother : $f(x,y)= x y^{3} + 2 \, x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 3 & 2 & 1 \\
0 & 0 & 0 & 0 \\
0 & 1 & 2 & 3
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x y^{3} + x y^{2} + 3  x y}}\makeatother : $f(x,y)= x y^{3} + x y^{2} + 3 \, x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 1 & 2 & 3 \\
0 & 2 & 0 & 2 \\
0 & 1 & 2 & 3
\end{array}\right)
$$

\subsection*{Class 13}
\noindent
\makeatletter\Hy@raisedlink{\hypertarget{class13}}\makeatother
Singular Values: $\vec{s}= \left(0.70711,\,0.5,\,0.5,\,0.0\right) $

\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x^{3} y + x y^{2}}}\makeatother : $f(x,y)= x^{3} y + x y^{2}$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 2 & 2 & 2 \\
0 & 2 & 0 & 2 \\
0 & 0 & 2 & 0
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x^{3} y + x^{2} y + x y^{2} + x y}}\makeatother : $f(x,y)= x^{3} y + x^{2} y + x y^{2} + x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 0 & 0 & 2 \\
0 & 2 & 0 & 2 \\
0 & 2 & 0 & 0
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x^{3} y + x y^{2} + 2  x y}}\makeatother : $f(x,y)= x^{3} y + x y^{2} + 2 \, x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 0 & 2 & 0 \\
0 & 2 & 0 & 2 \\
0 & 2 & 2 & 2
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x^{3} y + x^{2} y + x y^{2} + 3  x y}}\makeatother : $f(x,y)= x^{3} y + x^{2} y + x y^{2} + 3 \, x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 2 & 0 & 0 \\
0 & 2 & 0 & 2 \\
0 & 0 & 0 & 2
\end{array}\right)
$$

\subsection*{Class 14}
\noindent
\makeatletter\Hy@raisedlink{\hypertarget{class14}}\makeatother
Singular Values: $\vec{s}= \left(0.70711,\,0.5,\,0.5,\,0.0\right) $

\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x^{3} y}}\makeatother : $f(x,y)= x^{3} y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 1 & 0 & 3 \\
0 & 2 & 0 & 2 \\
0 & 3 & 0 & 1
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x^{3} y + x^{2} y + x y}}\makeatother : $f(x,y)= x^{3} y + x^{2} y + x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 3 & 2 & 3 \\
0 & 2 & 0 & 2 \\
0 & 1 & 2 & 1
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x^{3} y + 2  x y}}\makeatother : $f(x,y)= x^{3} y + 2 \, x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 3 & 0 & 1 \\
0 & 2 & 0 & 2 \\
0 & 1 & 0 & 3
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x^{3} y + x^{2} y + 3  x y}}\makeatother : $f(x,y)= x^{3} y + x^{2} y + 3 \, x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 1 & 2 & 1 \\
0 & 2 & 0 & 2 \\
0 & 3 & 2 & 3
\end{array}\right)
$$

\subsection*{Class 15}
\noindent
\makeatletter\Hy@raisedlink{\hypertarget{class15}}\makeatother
Singular Values: $\vec{s}= \left(0.5,\,0.5,\,0.5,\,0.5\right) $

\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x^{2} y + x y^{2}}}\makeatother : $f(x,y)= x^{2} y + x y^{2}$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 2 & 2 & 0 \\
0 & 2 & 0 & 2 \\
0 & 0 & 2 & 2
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x^{2} y + x y^{2} + 2  x y}}\makeatother : $f(x,y)= x^{2} y + x y^{2} + 2 \, x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 0 & 2 & 2 \\
0 & 2 & 0 & 2 \\
0 & 2 & 2 & 0
\end{array}\right)
$$

\subsection*{Class 16}
\noindent
\makeatletter\Hy@raisedlink{\hypertarget{class16}}\makeatother
Singular Values: $\vec{s}= \left(0.5,\,0.5,\,0.5,\,0.5\right) $

\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{x y}}\makeatother : $f(x,y)= x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 1 & 2 & 3 \\
0 & 2 & 0 & 2 \\
0 & 3 & 2 & 1
\end{array}\right)
$$


\noindent
Polynomial\makeatletter\Hy@raisedlink{\hypertarget{3  x y}}\makeatother : $f(x,y)= 3 \, x y$
$$
M_f = 
\left(\begin{array}{rrrr}
0 & 0 & 0 & 0 \\
0 & 3 & 2 & 1 \\
0 & 2 & 0 & 2 \\
0 & 1 & 2 & 3
\end{array}\right)
$$

==> docs/measurement.tex <==
In this subsection we study TEH-states after Local Pauli measurements and show equivalences of TEH states under such measurements. In particular, based on this we present a construction to {\it deterministically} produce a state that is LU equivalent to a TEH state.

%\colorbox{yellow}{NOTE (David)} The two following paragraphs can perhaps be shortened, by referring to the material in the partial trace subsection above.\colorbox{yellow}{END NOTE}

%Let us start with post-$Z$-measurement TEH states.
%\begin{definition}
%Given a TEH-state $\ket{G_f}$. If we write it as follows,
%\begin{equation}
%\ket{G_f}=\frac{1}{\sqrt{d}}\bigg(\ket{0}_a\ket{G_{f_0}}+\ket{1}_a\ket{G_{f_1}}+\dots +\ket{d-1}_a\ket{G_{f_{d-1}}}\bigg),
%\end{equation}
%we say that TEH-state is \emph{expanded over a vertex} $a\in V$.  By definition all $\ket{G_{f_{i}}}$'s are also TEH-states respectively corresponding to the post-measurement state for   
%$i$-th outcome of computational bases measurement on a vertex $a$.

%If we choose a subset of vertices $V_x\subset V$ instead of a vertex $a$, we say that TEH-state is expanded over a set of vertices $V_x\subset V$ and expansion is done iteratively for every vertex in $V_x$. Such expansions can also be used for qubit or qudit hypergraphs states.
%\end{definition}

To present more clearly the subsequent constructions, let us first look at a qubit case in the following Lemma: 
\begin{lemma}\label{lemma:qubitXmeasurement}\cite{2018arXiv180512093G} Given a qubit hypergraph state $\ket{H}$ corresponding to a hypergraph $H=(V,E)$ with more than three vertices, let us expand this hypergraph over vertices $a,b,c\in V$. If the expanded state can be written as 
\begin{equation}
    \ket{H}=\frac{1}{\sqrt{8}}\bigg[(\ket{000}+\ket{001}+\ket{010}+\ket{100})_{abc}\otimes \ket{H_\alpha}+(\ket{111}+\ket{110}+\ket{101}+\ket{011})_{abc}\otimes \ket{H_\beta}\bigg]
\end{equation}
and $\ket{H_\beta}=Z_i \prod_{{\bf e}}(CZ)_{\bf e}\ket{H_\alpha}$, 
where  $i\in V$ and $({\bf e})$ are indices referring to (qubit) hyperedges over the vertices $\hat{V}=V\backslash \{a,b,c,i\}$.
Measuring vertices $a,b,c$ in the $X$ (i.e., basis projects on a  state, which is LU equivalent to a hypergraph state.
\end{lemma}

When $X$ measurements are made on vertices $(a,b,c)$, a post-measurement state depending on measurement outcomes corresponds, up to a local Fourrier transform on qubit $i$, to one of the two equal superposition of two hypergraph states, i.e., $F_i(\ket{H_\alpha}\pm\ket{H_\beta})$ (where $F_i$ is the Fourrier transform defined in Eq.~(\ref{eq:FTdefinition}), acting on qubit $i$). Therefore, conditions on these equally-weighted superpositions of two hypergraphs $\ket{H_\alpha}$ and $\ket{H_\beta}$ are central here. 

We would like to generalize this construction to a higher dimensional case by expanding a higher dimensional TEH state over three or more qudits and deriving conditions for equal superposition TEH states to again give a TEH state. For this, we make use of the $d$-dimensional Fourrier transform $F$ defined in Eq.~(\ref{eq:FTdefinition}).

%This Hadamard operator is not Hermitian, but it is unitary. 
%If the computational bases corresponding to Pauli-$Z^{(d)}$ to be computational bases $\{\ket{i}\ |\ 0\leq i\leq (d-1)\}$, then measurement bases corresponding to Pauli-$X^{(d)}$ is given by $\{F\ket{i}\ |\ 0\leq i\leq (d-1)\}$.

%Then we are ready to formulate 
A sufficient criterion for equally-weighted superposition of qudit hypergraph states (with the edge function $E({\bf e})$ restricted as in Eq.~(\ref{eq:tradhypcond})) to be equivalent to a qudit hypergraph state (with the same restrictions on $E({\bf e})$) is:

\colorbox{yellow}{NOTE (Giuseppe)}
Perhaps a picture of the hypergraph in the following construction would be helpful
\colorbox{yellow}{END NOTE}


\begin{lemma}\label{Lemma:SuperpositionofHypergraphs}
Let $\ket{H_{0}}$, be $d$-dimensional hypergraph state 
defined by the hypergraph $H_{0}=(V,E)$ with $N$ vertices and with a certain edge function $E$ satisfying Eq.~(\ref{eq:tradhypcond}). Let then 
$\ket{H_{1}}$, $\ket{H_{2}}$, $\dots$ $\ket{H_{d-1}}$ be $d$-dimensional hypergraph states, such that the corresponding hypergraphs are
H_1=(V,E\cup \{a\} \cup\Tilde{E})$, $H_2^{(d)}=(V,E\cup \{a\}\cup \{a\} \cup\Tilde{E}\cup\Tilde{E})$, $\dots$ $H_{d-1}^{(d)}=(V,E\cup \{a\}\cup \dots \cup \{a\} \cup \Tilde{E} \cup\dots \cup\Tilde{E})$, where $a \in V$ and $a$ is not contained in any hypergedge in $\Tilde{E}$. Write hyperedges of $H_0$ as $E=\Tilde{E}_0\cup E'$, where $E'$ are hyperedges containing a vertex $a$.  If for every $e'\in E'$ and $\Tilde{e}\in \Tilde{E}$, $e'\cap\Tilde{e}_0=\emptyset$, then the superposition $\sum_{i=0}^{d-1}\ket{H^{(d)}_i}$ again gives a hypergraph state up to a Hadamard gate $F_a$ acting on a vertex $a$:
\begin{equation}
F_a\bigg(\sum_{i=0}^{d-1}\ket{H_i}\bigg)\propto \prod_{\Tilde{e}_0\in \Tilde{E}_0}(CZ)_{\bf \Tilde{e}_0}\prod_{\Tilde{e}\in \Tilde{E}}(CZ)_{\bf \Tilde{e}\cup \{a\}}\prod_{e'\in E'}(CZ)^{d-1}_{\bf \Tilde{e}\cup e'} \ket{+}^{\otimes N}.
\end{equation}
\end{lemma}

The detailed proof is in Appendix~\ref{app:D}.






%\begin{align}
 %   F_1\sum_{i=0}^{d-1}\ket{H^{(d)}_i}= & \  F_1\bigg(\ket{H^{(d)}_0}+\sum_{i=1} ^{d-1}Z_1^i\prod_{\Tilde{e}\in \Tilde{E}}C^i_{\Tilde{e}}\ket{H^{(d)}_0}  \bigg)\label{Eq:superpositionProof_1}\\
  %  =& \ H_1^{(d)}\prod_{e\in E}C_{e}\bigg(\ket{+}^{\otimes N}+\sum_{i=1}^{d-1}Z^{i}_1 \prod_{\Tilde{e}\in \Tilde{E}}C^i_{\Tilde{e}}\ket{+}^{\otimes N}\bigg)\label{Eq:superpositionProof_2}\\
   % =& \ H_1^{(d)}\prod_{e\in E}C_{e}\Bar{H}_1^{(d)}H_1^{(d)}\bigg(\ket{+}_1+\sum_{i=1}^{d-1}Z^{i}_1\ket{+}_1\prod_{\Tilde{e}\in \Tilde{E}}C^i_{\Tilde{e}}\bigg) \ket{+}^{\otimes N-1}\label{Eq:superpositionProof_3}\\
%    =& \ H_1^{(d)}\prod_{e\in E}C_{e}\Bar{H}_1^{(d)}\bigg(\sum_{i=0}^{d-1}\ket{i}_1\prod_{\Tilde{e}\in \Tilde{E}}C^i_{\Tilde{e}}\bigg) \ket{+}^{\otimes N-1}\label{Eq:superpositionProof_4}\\
 %   \propto &\  H_1^{(d)}\prod_{\Tilde{e}_0\in \Tilde{E}_0}C_{\Tilde{e}_0}\prod_{e'\in E'}C_{e'}\Bar{H}_1^{(d)}\prod_{\Tilde{e}\in \Tilde{E}}C_{\Tilde{e}\cup \{1\}} \ket{+}^{\otimes N}\label{Eq:superpositionProof_5}\\
%     =& \ \prod_{\Tilde{e}_0\in \Tilde{E}_0}C_{\Tilde{e}_0}H_1^{(d)}\prod_{e'\in E'}C_{e'}\Bar{H}_1^{(d)}\prod_{\Tilde{e}\in \Tilde{E}}C_{\Tilde{e}\cup \{1\}} \ket{+}^{\otimes N}\label{Eq:superpositionProof_6}\\
    % =& \ \prod_{\Tilde{e}_0\in \Tilde{E}_0}C_{\Tilde{e}_0}\prod_{e'\in E'}CNOT_{e'\backslash\{1\},1}\prod_{\Tilde{e}\in \Tilde{E}}C_{\Tilde{e}\cup \{1\}} \ket{+}^{\otimes N}\label{Eq:superpositionProof_7}\\
    %  =& \ \prod_{\Tilde{e}_0\in \Tilde{E}_0}C_{\Tilde{e}_0}\prod_{\Tilde{e}\in \Tilde{E}}C_{\Tilde{e}\cup \{1\}}\prod_{e'\in E'}C^{d-1}_{\Tilde{e}\cup e'} \ket{+}^{\otimes N}
%\end{align}


As a consequence, we have the following 

\begin{corollary}
Respecting all the conditions for hypergraph states in Lemma \ref{Lemma:SuperpositionofHypergraphs}, superposition of the type $\sum_{i=0}^{d-1}\omega^{k \cdot i}\ket{H_i}$, for all $1\leq k \leq (d-1)$  also gives states LU equivalent to  a hypergraph state:

\begin{equation}
F_1\bigg(\sum_{i=0}^{d-1}\omega^{k \cdot i}\ket{H_i}\bigg)\propto Z_1^{k}\prod_{\Tilde{e}_0\in \Tilde{E}_0}(CZ)_{\bf \Tilde{e}_0}\prod_{\Tilde{e}\in \Tilde{E}}(CZ)_{\bf \Tilde{e}\cup \{a\}}\prod_{e'\in E'}(CZ)^{d-1}_{\bf \Tilde{e}\cup e'}(CZ)^{k(d-1)}_{\bf e'} \ket{+}^{\otimes N}.
\end{equation}
\end{corollary}


Having investigated superposition rules for qudit hypergraph states, we now investigate a similar construction to the one in Lemma \ref{lemma:qubitXmeasurement} but for qudits. 

For simplicity we consider a qutrit graph state $\ket{G}$ case, but the results also hold for arbitrary local dimension $d$. We assume that the corresponding graph $G=(V,E)$ is connected. We can expand this state over a vertex $1$:
\begin{equation}
    \ket{G}\propto\ket{0}_1 \ket{G_0}+\ket{1}_1 \ket{G_1}+\ket{2}_1 \ket{G_2}.
\end{equation}
Then by definition  $\ket{G_i}$'s are also graph states and they correspond to the outcome $\ket{i}$ of a Pauli-$Z$ bases measurement.
However, if we measure the state in the Pauli-$X$ basis, we need to check whether the conditions of Lemma \ref{Lemma:SuperpositionofHypergraphs} are satisfied. 
In qubit graph states Pauli-$X$ basis measurements always project onto qubit graphs states up to a local Clifford correction \colorbox{yellow}{[CITE]}. 
However, already in the qutrit graph state case the Pauli-$X$ measurement projects on a general TEH state (and not a graph state, which we would like). 
We shall note that the post-measurement state is local unitary (not local Clifford) equivalent to a qudit graph state. 

To illustrate this, we consider a simple three qutrit example
$\ket{G}=Z_{12}Z_{13}Z_{23}\ket{+}^{\otimes 3}$, where the first qutrit is measured in Pauli-$X$ basis. Then, the resulting state does not obey the conditions in Lemma \ref{Lemma:SuperpositionofHypergraphs} and by a direct inspection we can check that, e.g., in case of outcome $\bra{+}_1$, it gives as post-measurement state, up to a Hadamard gate on vertex $2$:   
\begin{equation}
\Tilde{Z}^2_3 Z_{23}\ket{+}^{\otimes 3},
\end{equation}
where $\Tilde{Z}=\ketbra{0}+\omega \ketbra{1}+\omega \ketbra{2}$.

Therefore, the resulting state is a TEH-state but it is LU equivalent to a qutrit graph state. 

Similarly one can find more complicated examples of qudit hypergraph states where only one qudit is measured in Pauli-$X$ bases and the resulting state is either a hypergraph state again or a TEH-state, but not necessarily locally equivalent to a qudit graph state. 
Besides, if only one qudit is measured, our sufficient criterion is only applied to the cases when a measured vertex is only included in graph edges  and not in any hyperedges, which is not the most general case.
\colorbox{yellow}{A simple but a nice example will be added here.}

So, we restrict ourselves to qudit hypergraphs states with three or higher cardinality edges, similar to the qubit case \cite{2018arXiv180512093G} and we are interested in possible constructions such that the expansion of the state over more than one qudits satisfies Lemma \ref{Lemma:SuperpositionofHypergraphs} (similarly to the Lemma \ref{lemma:qubitXmeasurement}).  

Let us again restrict ourselves to the qutrit case for simplicity and then generalize results. 

\begin{lemma}
Given a three or four-qutrit connected hypergrpah state $\ket{H}$ with hyperedges of minimal cardinality three, corresponding to a hypergraph $H=(V,E)$ . There is no vertex or number of vertices $|V|-2$, such that they can be measured in Pauli-$X$ basis and a resulting states satisfy the equal superposition requirements of Lemma \ref{Lemma:SuperpositionofHypergraphs}.
\end{lemma}
\begin{proof}
For $|V|=3$, the statement is trivial. The only possible hyperedges are $E=\{\{1,2,3\}\}$ or $E=\{\{1,2,3\}\}$,
\colorbox{yellow}{NOTE (giuseppe) I think there is a typo here: the same hyperedge is repeated?} expanding it over one vertex %only 
cannot give hypergraphs satisfying  \ref{Lemma:SuperpositionofHypergraphs}. Indeed expanding only over one vertex can never do the job.

The proof is slightly more involving for four qutrits. We have to expand the state over two vertices. For this we divide all computational basis elements for two vertices in three groups:
\begin{align}
\begin{split}
   \ket{H}\propto &\  \bigg(\ket{00}+\ket{01}+\ket{02}+\ket{10}+\ket{20}\bigg)\otimes \ket{H_0}\\
   + &\ \bigg(\sum_{x}\ket{x}\bigg)\otimes Z_3\otimes Z_4 \ket{H_0}\\
   + &\ \bigg(\sum_{y}\ket{y}\bigg)\otimes Z^2_3\otimes Z^2_4 \ket{H_0},
\end{split}    
\end{align}
where $\sum_{x}\ket{x}+\sum_{y}\ket{y}=\ket{11}+\ket{12}+\ket{21}+\ket{22}$ are computational basis elements.  Since there are no graph edges in hypergraph $H$, the first group in the expansion must contain five computational basis elements which have at most one non-zero entry. Then there are only $3^2-5=4$ computational bases elements left to be assigned to one of the two groups. By definition of a qutrit hypergraph state, the group which contains $\ket{11}$ must contain $\ket{22}$ as well and the other group must countain $\ket{12}$ and $\ket{21}$. Without loss of generality we assign $\sum_{x}\ket{x}=\ket{11}+\ket{22}$. 

Then, if measurement results on first and second vertices are $\bra{+}\bra{+}$ one can directly inspect that the post measurement state is of the form:
\begin{equation}
\bra{+}_1\bra{+}_2\ket{H}\propto\bigg( 5 \mathbbm{1}\otimes\mathbbm{1}+2 Z_3\otimes Z_4 +2Z^2_3\otimes Z^2_4 \bigg)\ket{H_0}.
\end{equation}
Since the hypergraphs have different weights they are not equivalent to a two qutrit graph state.
\end{proof} 

The results can be directly generalized for arbitrary $d$: There are $d^2$ computational basis elements in total, which need to be distributed equally in $d$ groups but the first group must contain $(2d-1)$ elements. 

\begin{lemma}
Given a five-qutrit connected hypergrpah state $\ket{H}$ with hyperedges of minimal cardinality three. There is no vertex or number of vertices, such that they can be measured in Pauli-$X$ basis and a resulting two-qutrit state satisfies the  equal superposition requirements of Lemma \ref{Lemma:SuperpositionofHypergraphs}.
\end{lemma}
\begin{proof}
The proof goes along the line to the proof of the previous Lemma. We shall expand the hypergraph over three vertices. This gives us $3^3=27$ computational basis elements, which we must evenly distribute in three different groups:
\begin{align}
    \ket{H}\propto &\ \bigg(\sum_u \ket{u}\bigg)\otimes \ket{H_0)}\\
    + &\ \bigg(\sum_v \ket{v}\bigg)\otimes Z_4\otimes Z_5 \ket{H_0)}\\
    + &\ \bigg(\sum_w \ket{w}\bigg)\otimes Z^2_4\otimes Z^2_5 \ket{H_0)}.
\end{align}
Due to the cardinality of the hyperedge of the original hypergraph state, we must assign to the first group the following seven elements: 
\begin{equation}
    \ket{000},\ket{001},\ket{002},\ket{010},\ket{020},\ket{100},\ket{200}.
\end{equation}
There seems to be a lot of freedom on how to assign the rest of $20$ remaining elements. However, %with the 
by exhaustive search one can find that there is no way to group all the computational basis elements in three groups compatible with all the requirements of %the 
Lemma \ref{Lemma:SuperpositionofHypergraphs} and the definition of qutrit hypergraph state. 
\end{proof}

If we relax the requirement for the original state to be a qudit hypergraph state, in analogy with the qubit case in Lemma \ref{lemma:qubitXmeasurement}, we can find an expansion of a five-qutrit TEH state, which can be deterministically projected on either another TEH state or a qudit hypergraph state:    


\begin{lemma}\label{lemma:TEHbox} The following five qutrit TEH-state can be deterministically projected on a hypergraph state after Pauli-$X$ %bases 
measurements on the first three qutrits:
\begin{align}
    \begin{split}
        \ket{G_f}\propto(\ket{000}+\ket{001}+\ket{002}+\ket{010}+\ket{020}+\ket{100}+\ket{200}+\ket{012}+\ket{021}) &\otimes \ket{H_0}\\
        + \ (\ket{111}+\ket{011}+\ket{101}+\ket{110}+\ket{112}+\ket{121}+\ket{211}+\ket{102}+\ket{120}) & \otimes \ket{H_1}\\
        + \ (\ket{222}+\ket{022}+\ket{202}+\ket{220}+\ket{122}+\ket{212}+\ket{221}+\ket{201}+\ket{210}) & \otimes \ket{H_2},
    \end{split}
\end{align}
as long as the hypergraphs $H_0$, $H_1$, and $H_2$ satisfy the conditions of Lemma \ref{Lemma:SuperpositionofHypergraphs}.  
\end{lemma}

\begin{proof}
We prove this statement by direct inspection. It is sufficient to show that regardless of the measurement outcomes for the first three qutrits, the possible post-measurement state is always an equally-weighted superposition of the qudit hypergraph states $\ket{H_0},\ket{H_1},$ and $\ket{H_2}$. Note that the particles $2$ and $3$ are permutationally symmetric, which reduces number of possibilities. 
See Table \ref{table:outcomes} in the Appendix for the exact correspondence between  measurement outcomes and post-measurement states.
\end{proof}

Finally, we can generalize the previous Lemma to the arbitrary local dimensional case. The key observation to make in qubit and qutrit cases is that computational baseis elements assigned to the first group entirely determine the elements assigned to the rest of the groups. They differ only by application of Pauli-$X$ unitaries on all parties. For the qutrit case, we apply $X^{\otimes 3}$ twice to get the computational basis elements of the third group. We use the same techniques for arbitrary local dimension $d$. For convenience we define the following sum of computational bases elements 
\begin{align}
    \ket{S} = & \ket{001} + \dots + \ket{00(d-1)}+\ket{010} + \dots + \ket{0(d-1)0}+\ket{100} + \dots + \ket{(d-1)00}\\
    +& \ket{000} + \sum_{i\neq j >0}^{d-1}\ket{0ij}. 
\end{align}

\begin{prop}\label{lemma:TEHdbox} The following five qudit TEH state can be deterministically projected onto a hypergraph state after Pauli-$X$ %bases 
measurements on first three qudits:
\begin{equation}
    \ket{G_f}\propto \ket{S} \ket{H_0}+ X_1 \otimes X_2\otimes X_3\ket{S} \ket{H_1}+\dots+X^{d-1}_1 \otimes X^{d-1}_2\otimes X^{d-1}_3\ket{S} \ket{H_{d-1}},
\end{equation}
as long as the hypergraphs $H_0$, $H_1,\dots, H_{d-2}$, and $H_{d-1}$ satisfy the conditions of Lemma \ref{Lemma:SuperpositionofHypergraphs}.
\end{prop}

\begin{proof}
First of all it is easy to see that $\ket{G_f}$ is indeed a TEH-state. Let us denote $\ket{e_i}$'s to be effects of the Pauli-$X$ %bases 
measurements for $0 \leq i\leq (d-1)$. Then for any $0 \leq i,j,k,l \leq (d-1)$ the following holds: 
\begin{align}
    \bra{e_i}\bra{e_j}\bra{e_k} X^l_1\otimes X^l_2 \otimes X^l_3 \ket{S}= & \bra{e_0}\bra{e_0}\bra{e_0} Z^i_1 X^l_1\otimes Z^j_2 X^l_2 \otimes Z^k_3 X^l_3 \ket{S}\\
    = \omega ^{-(i+j+k)l} &  \bra{e_0}\bra{e_0}\bra{e_0}X^l_1 Z^i_1 \otimes X^l_2 Z^j_2  \otimes X^l_3 Z^k_3  \ket{S}\\
    = \omega ^{-(i+j+k)l} &  \bra{e_0}\bra{e_0}\bra{e_0} Z^i_1 \otimes  Z^j_2  \otimes  Z^k_3  \ket{S}\\
    = \omega ^{-(i+j+k)l} &  \bra{e_i}\bra{e_j}\bra{e_k} \ket{S}.
\end{align}
Therefore, for all $l,i,j,k$, from the linearity we get that  $\bra{e_i}\bra{e_j}\bra{e_k}\ket{G_f}$  always projects on an equal weighted superposition of hypergraph states $\ket{H_l}$.
\end{proof}

In the applications section we show that whenever the particular hypergraph states $\ket{H_0},\dots$ $\ket{H_{d-1}}$ \colorbox{yellow}{NOTE (giuseppe) This sentence looks incomplete}, the TEH-state is useful for measurement-based quantum computation.


==> docs/stabilizer.tex <==
\noindent 
In this section, we construct stabilizers for FFE states. 
In particular, we make use of finite-function-encoding Pauli operations to generalize the Pauli stabilizer formalism for hypergraph states \cite{1367-2630-15-11-113022,2017PhRvA..95e2340S}.
We present a construction of a stabilizer set that uniquely determines an arbitrary FFE state, and we show that a property
called \emph{internal commutativity} is satisfied if and only if the FFE state can be obtained with local finite-function-encoding Pauli operations from the qudit hypergraph states defined in Ref.~\cite{2017PhRvA..95e2340S}.

Recall that graph states are determined by a discrete Abelian group of local Pauli operators, generated by $X_i\bigotimes_{j\neq i} Z_j$, where  $X_i$ and $Z_j$ are local operators  acting on the $i$-th and $j$-th subsystem. 
Hypergraph states are also determined by an Abelian discrete group of stabilizers of a similar form, but this time, with controlled-$Z$ operators, which are no longer local \cite{1367-2630-15-11-113022,2017PhRvA..95e2340S}, but still commute with the $X$ operators. 
Here, we show that FFE states are also determined by Abelian groups of operators having a similar form, but in general the finite-function-encoding Pauli $Z$ operators will not commute with the $X$ operators. 
The latter {\it internal commutativity}, as we are going to prove, is satisfied only for a special class of FFE states, that are LFP equivalent to the qudit hypergraph states. 

Given a function $f\colon \mathds{Z}_d^n \bl{\to} \mathds{Z}_d$ and a $n$-$d$it permutation $\pi\colon \mathds{Z}^n_d\bl{\to} \mathds{Z}^n_d$, let $S_{f,\pi}$ denote the operator 
\begin{equation}\label{def:stabilizer}
S_{f,\pi}=X_{\pi}Z_{f\circ \pi -f}.
\end{equation}
It is straightforward to check that $S_{f,\pi}$ stabilizes $\ket{f}$, that is
\[
S_{f,\pi} \ket{f} = \ket{f}.
\]
For a fixed $f$, these $(d^n)!$ operators $S_{f,\pi}$ (over all $(d^n)!$ permutations $\pi$ of $n$-$d$its) constitute the \bl{FP} stabilizer group of $\ket{f}$. This group is not Abelian, but it has some useful Abelian subgroups. 
In particular, we will show that there is an Abelian subgroup of \bl{FP} stabilizers with the property that the FFE state from which they are constructed is the unique simultaneous $+1$-eigenstate of the set of $n$ generators of the subgroup.
It is easy to see that $S_{f,\pi}$ and $S_{f,\sigma}$ commute whenever $\pi$ and $\sigma$ commute. 
In particular, $S_{f,\pi_i},S_{f,\sigma_j}$, where the permutations act on different qudits always commute.
If we fix \bl{an arbitrary} $d$-cycle ${\kappa_i}$ for each \bl{subsystem} $i$, the set of operators $\{ S_{f,\kappa_i}\}_{i=1}^n$ uniquely determines $\ket{f}$, among all $n$-qudit states, as their simultaneous $+1$-eigenstate. 

\begin{prop}\label{cyclestabunique}
The state $\ket{f}$ is the unique simultaneous $+1$-eigenvector of the set of $n$ FP operators $\{ S_{f,\kappa_i}\colon 1\leq i\leq n\}$, where for each $i$, $\kappa_i$ is a $d$-cycle.
\end{prop}
The proof can be found in Appendix~\ref{appendixA}.
In the above construction, the choice of the $d$-cycles $\kappa_i$ is left as a free parameter.

Now, we are interested in another property of the stabilizers: \emph{internal commutativity}.
In other words, we are interested to find a family of stabilizing operators that determine a state $\ket{f}$ uniquely and also \emph{internally 
commute}, i.e., $
X_{\kappa_i}Z_{f\circ\kappa_{i} - f}
=Z_{f\circ\kappa_{i} - f}X_{\kappa_i}
\;\forall i$. 
This will be done by looking at the previous construction and studying which functions give rise to internally commuting stabilizing operators:

\begin{lemma}
\label{lem:commutativity_cyclic_permutation}
Let $\kappa$ be a $d$-cycle. Then $X_{\kappa_i}Z_h = Z_hX_{\kappa_i}$ if and only if $h(\vec{x})$ does not depend on the value of $x_i$.
%In this case we can also write
%$X_{\kappa_i} Z_h=X_{\kappa_i}\otimes Z_h$.

\end{lemma}
\begin{proof}
\bl{From the left hand side of}{} the general commutativity relation \eqref{XZ_commutation},
\begin{align}\label{eq:commutativityofhandhkappa}
   X_{\kappa_i}Z_h &= Z_h X_{\kappa_i}\Longleftrightarrow h\circ\kappa_i(\vec{x}) = h(\vec{x}).
\end{align}
This implies  
\[
\forall c\in\Fd: h(x_1,\dots,x_{i-1},c,x_{i+1},\dots,x_n) = h(x_1,\dots,x_{i-1},\kappa_i(c),x_{i+1},\dots,x_n),
\]
which, together with  $\kappa_i$ being a $d$-cycle, implies that $h$ is independent of $x_i$.
In particular, we have that $X_{\kappa_i}$ and $Z_h$ act non-trivially on the Hilbert spaces of different parties, and we can write their product in a tensor product form.
\end{proof}

Due to this, it turns out that internally commuting stabilizers exists only for a subset of functions: 

\begin{prop}
\label{prop:internally_commuting}
Let $\left\{S_{f,\kappa_i}\right\}_{i=1}^n$ be a set of stabilizers which uniquely determines a state $\ket{f}$ and let the $\kappa_i=\pi_i^{-1}\kappa_i^{+}\pi_i$ be fixed $d$-cycles.
The stabilizers $S_{f,\kappa_i}=X_{\kappa_i}Z_{f\circ\kappa_{i} - f}$ commute internally if and only if the function $f$ can be written as 
\begin{equation}
  f=f^\prime \circ \pi_1\circ \dots \circ \pi_n,
\end{equation}
where $f^\prime$ has degree at most $1$ in each variable.
\end{prop}
The proof can be found in the Appendix~\ref{appendixA}. 
This result shows, that functions that have degree at most $1$ in each variable indeed have a special property that is lost in the case of general FFE states.  
Those are precisely LFP (and hence LU) equivalent to the qudit hypergraph states defined in Ref.~\cite{2017PhRvA..95e2340S} (see also table \ref{table:graphcomparisons} and the discussion above it). 
Thus, the latter have stabilizers with a simpler structure than those of general FFE states. 
Nevertheless, the above construction is still a direct generalization of the qubit stabilizers formalism and one can still recover a similar structure. 
For example, as an additional minor result we present in Appendix~\ref{app:FFEwithContST} a family of states having continuous unitary stabilizers, with a construction that generalizes that of Ref.~\cite{PhysRevA.79.042318,hypergraph2014}. 
